Context-Aware Group Captioning via Self-Attention and Contrastive Features

While image captioning has progressed rapidly, existing works focus mainly on describing single images. In this paper, we introduce a new task, context-aware group captioning, which aims to describe a group of target images in the context of another group of related reference images. Context-aware group captioning requires not only summarizing information from both the target and reference image group but also contrasting between them. To solve this problem, we propose a framework combining self-attention mechanism with contrastive feature construction to effectively summarize common information from each image group while capturing discriminative information between them. To build the dataset for this task, we propose to group the images and generate the group captions based on single image captions using scene graphs matching. Our datasets are constructed on top of the public Conceptual Captions dataset and our new Stock Captions dataset. Experiments on the two datasets show the effectiveness of our method on this new task. Related Datasets and code are released at https://lizw14.github.io/project/groupcap .

==> experiments.tex <==
%\setlength{\tabcolsep}{0.08cm}
\newcolumntype{M}{>{\centering\arraybackslash}X}
\begin{table*}[h!]
\small{
%\small{
  \begin{center}
    %\begin{tabular}{|l|C{\colwidthA}|C{\colwidthA}|C{\colwidthA}|C{\colwidthA}|C{\colwidthA}|C{\colwidthA}|C{\colwidthA}|}
    %\begin{tabular}{|l{2cm}|C{\colwidthA}|C{\colwidthA}|C{\colwidthA}|C{\colwidthA}|C{\colwidthA}|C{\colwidthA}|C{\colwidthA}|}
    \begin{tabularx}{0.8\textwidth}{|l|MMMMMMM|}
        \hline
         & {WordAcc} & {CIDER} & {WER} & {BLEU1} & {BLEU2} & {METEOR} & {ROUGE}\\
        \hline
        \multicolumn{8}{|c|}{Conceptual}\\
        % {-} & {WordAcc} & {CIDER} & {WER} & {BLEU1} & {BLEU2} & {METEOR} & {ROUGE}\\
        %\hline
        %\multicolumn{8}{|c|}{\textbf{Conceptual}}\\
        \hline
        {Average} & 36.7329 & 1.9591 & 1.6859 & 0.4932 & 0.2782 & 0.3956 & 0.4964 \\
        % \textbf{Atten20} & 36.1231 & 2.0727 & 1.6851 & 0.5044 & 0.2976 & 0.4089 & 0.5059 \\
        {SA} & 37.9916 & 2.1446 & 1.6423 & 0.5175 & 0.3103 & 0.4224 & 0.5203 \\
        % \textbf{SA+CA} & 36.2892 & 2.1282 & 1.6697 & 0.5041 & 0.3094 & 0.4145 & 0.5062 \\
        %\textbf{SA+NCA} & 37.6046 & 2.2109 & 1.6344 & 0.5155 & 0.3183 & 0.4237 & 0.5165 \\
        % \textbf{SA+tgt-ref} & 38.2574 & 2.1499 & 1.6332 & 0.5213 & 0.3106 & 0.4228 & 0.5203 \\
        % \textbf{SA+tgt-avg} & 38.5916 & 2.1821 & 1.6230 & 0.5218 & 0.3156 & 0.4261 & 0.5229 \\
        {Average+Contrast} & 37.8450 & 2.0315 & 1.6534 & 0.5007 & 0.2935 & 0.4057 & 0.5027 \\
        \textbf{SA+Contrast} & \textbf{39.4496} & \textbf{2.2917} & \textbf{1.5806} & \textbf{0.5380} & \textbf{0.3313} & \textbf{0.4405} & \textbf{0.5352} \\
        \hline
        \multicolumn{8}{|c|}{Stock}\\
        \hline
        {Average} & 37.9428	& 1.9034 & 1.1430 & 0.5334 & 0.2429 & 0.4042 & 0.5318 \\
        % \textbf{Atten20} & 38.9215 & 2.0271 & 1.0904 & 0.5451 & 0.2578 & 0.4166 & 0.5428 \\
        {SA} & 39.2410 & 2.1023 & 1.0829 & 0.5537 & 0.2696 & 0.4243 & 0.5515 \\
        % \textbf{SA+CA} & 38.6316 & 2.0414 & 1.0894 & 0.5440 & 0.2579 & 0.4139 & 0.5417 \\
        %\textbf{SA+NCA} & 39.3278 & 2.0833 & 1.0704 & 0.5490 & 0.2664 & 0.4207 & 0.5459 \\
        % \textbf{SA+tgt-ref} & 39.9114 & 2.1006 & 1.0699 & 0.5553 & 0.2731 & 0.4271 & 0.5523 \\
        % \textbf{SA+tgt-avg} & 40.2068 & 2.1115 & 1.0620 & 0.5537 & 0.2725 & 0.4262 & 0.5516 \\
        {Average+Contrast} & 39.1985 & 2.0278 & 1.0956 & 0.5397 & 0.2632 & 0.4139 & 0.5375\\
        \textbf{SA+Contrast} & \textbf{40.6113} & \textbf{2.1561} & \textbf{1.0529} & \textbf{0.5601} & \textbf{0.2796} & \textbf{0.4332} & \textbf{0.5572} \\
        \hline
        \end{tabularx}
  \end{center}
  \caption{Group captioning performance on the Conceptual Captions and Stock Captions dataset.}
  \label{tab:results}
%  }
}
\end{table*}

In this section, we first describe our evaluation results on the two datasets. 
Then we provide quantitative analysis and visualization to expose the effectiveness of 
different components of our model.

%% double column version
%\begin{table*}[h!]
%\small{
%  \begin{center}
%    \begin{tabular}{|l|r|r|r|r|r|r|r|}
%        \hline
%        \textbf{Model} & \textbf{WordAcc} & %\textbf{CIDER} & \textbf{WER} & %\textbf{BLEU1} & \textbf{BLEU2} & %\textbf{METEOR} & \textbf{ROUGE}\\
%        \hline
%        \textbf{Tgt0 + Ref15} & 24.4709 & 1.0399 & %1.4138 & 0.3891 & 0.0614 & 0.2341 & 0.3965 %\\
%        \textbf{Tgt1 + Ref15} & 28.7479 & 1.3447 & %1.3104 & 0.4375 & 0.1292 & 0.2938 & 0.4415 %\\
%        \textbf{Tgt3 + Ref15} & 34.6574 & 1.7641 & %1.1874 & 0.5045 & 0.2098 & 0.3698 & 0.5048 %\\
%        \textbf{Tgt5 + Ref0} & 31.8061 & 1.6767 & %1.2539 & 0.4600 & 0.2095 & 0.3475 & 0.4552 %\\
%        \textbf{Tgt5 + Ref15} & 40.6113 & 2.1561 & %1.0529 & 0.5601 & 0.2796 & 0.4332 & 0.5572 %\\
%    \hline
%        \end{tabular}
%  \end{center}
%  \caption{Experiment results when varying the %number of target and reference images. (Stock %dataset)}
%  \label{tab:number}
%  }
%\end{table*}

\begin{figure}
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\includegraphics[width=0.48\textwidth]{figures/4_atten.pdf}
\end{center}
   \caption{Visualization of $5\times5$ self-attention weight matrix for target image group. Each row sums up to 1. For group (a) \texttt{woman with balloon}, image 2 and image 3 are representative. For group (b) \texttt{yoga on beach}, image5 is representative. Images with more distinguishable features become the representative images of a group and get higher attention weights.}
\label{fig:attention}
\end{figure}


\setlength{\tabcolsep}{0.1cm}
\begin{table}
\footnotesize{
  \begin{center}
    \begin{tabular}{|l|r|r|r|r|r|}
        \hline
        {Model} & {WordAcc} & {CIDER} & {BLEU2} & {METEOR} & {ROUGE}\\
        \hline
        {Tgt0 + Ref15} & 24.4709 & 1.0399 & 0.0614 & 0.2341 & 0.3965 \\
        {Tgt1 + Ref15} & 28.7479 & 1.3447 & 0.1292 & 0.2938 & 0.4415 \\
        {Tgt3 + Ref15} & 34.6574 & 1.7641 & 0.2098 & 0.3698 & 0.5048 \\
        {Tgt5 + Ref0} & 31.8061 & 1.6767 & 0.2095 & 0.3475 & 0.4552 \\
        \textbf{Tgt5 + Ref15} & \textbf{40.6113} & \textbf{2.1561} & \textbf{0.2796} & \textbf{0.4332} & \textbf{0.5572} \\
    \hline
        \end{tabular}
  \end{center}
  \caption{Performance with varying the number of target and reference images. (evaluated on Stock Captions dataset)}
  \label{tab:number}
  }
\end{table}

%\subsection{Evaluation Metrics and Parameter Setting}
\subsection{Group Captioning Performance}

We evaluate our context-aware group captioning method on both Conceptual Captions and Stock Captions datasets. The same hyper-parameters are used for all experiments on each dataset. On the Stock Captions dataset, we use batch size 512 and initial learning rate $1\times10^{-4}$. On the Conceptual Captions dataset, we use batch size 512 and learning rate $5\times10^{-5}$. We train the model for 100 epochs with Adam optimizer\cite{kingma2014adam} on both datasets. 

We measure the captioning performance on the test splits in both datasets using a variety of captioning metrics. Specifically, we consider the standard metrics widely used in image captioning literature, including BLEU\cite{papineni2002bleu}, CIDER\cite{vedantam2015cider}, METEOR\cite{banerjee2005meteor} and ROUGE\cite{lin2004rouge}. In addition, since group descriptions are often short and compact, we put more emphasis on single word accuracy compared to traditional image captioning. We thus consider two additional metrics,  Word-by-word accuracy(WordAcc), word error rate(WER), that specifically assess word-based accuracy\footnote{Here we consider position-specific word accuracy. For example, prediction \emph{woman with straw hat} with ground truth \emph{woman with cowboy hat} has accuracy 75\%, while prediction \emph{woman with hat} has accuracy 50\%.}. 
%\lm{we many need to briefly explain how these are computed.} 
We also note that as some group descriptions may contain as few as two words, we do not consider BLEU3 and BLEU4 scores which evaluates tri-grams and 4-grams. 

%Common image caption evaluation metrics as well as single word metrics are used for evaluation. Since our group descriptions are short and compact, we put more emphasis on single word accuracy compared to traditional image captioning. While BLEU\cite{papineni2002bleu}, CIDER\cite{vedantam2015cider}, METEOR\cite{banerjee2005meteor} and ROUGE\cite{lin2004rouge} focus on evaluating consecutive word sequence quality, Word-by-word accuracy(WordAcc), word error rate(WER) focus on single words. Because the shortest descriptions contain only 2 words, BLEU3 and BLEU4 scores which evaluates tri-grams and 4-grams are not used. 

%\subsection{Results and analysis}
The captioning performance on the testing set of Conceptual Captions and Stock Captions datasets are reported in Table \ref{tab:results}. 
%In general, the self-attention and contrastive features individually, and collectively provide significant performance boost in both datasets across all performance measures.
Compared to aggregating features by averaging (\textbf{Average}, as in Section \ref{sec:baseline}), self-attention (\textbf{SA}) is more effective in computing group representation and leads to significant performance improvement. 
On top of feature aggregation, contrastive feature is critical for the model to generate context-aware caption which emphasizes the difference of target image group on context of reference group. Applying contrastive features (\textbf{Contrast}) to either feature aggregation methods leads to performance boost (\textbf{Average+Contrast, SA+Contrast}). To this end, our full model, which combines self-attention for group aggregation and contrastive feature for group comparing performs best, achieving 39.4\% WordAcc on Conceptual Captions and 40.6\% on Stock Captions. %\todo{Make this part more specific: emphasize that contrastive feature construction is critical. Adding that to the baseline Average which uses simple aggregation can significantly improve the performance. Similarly, using self-attention enables better feature aggregation and leads to performance boost over the baseline. Finally, combining two components to our full model lead to the best performance.}


\subsection{Discussion}

\begin{figure*}[h!]\vspace{-0.05in}
\begin{center}
%\fbox{\rule{0pt}{4in} \rule{.9\linewidth}{0pt}}
\includegraphics[width=0.99\linewidth]{figures/4_exp1_ver2.pdf}
\end{center}
   \caption{Qualitative prediction examples on Conceptual Captions (top row) and Stock Captions (bottom row) datasets. In each example, images in first row (in orange boxes) are target images while second to fourth rows (in blue boxes) are reference images. Our model can effectively summarize relevant information in the image groups during captioning. Our model also effectively takes discriminative information between the target and reference group into account during captioning to predict accurate group captioning results.}\vspace{-0.1in}
\label{fig:example}
\end{figure*}

\paragraph{Effectiveness of self-attention on feature aggregation.}
%Self-attention (\textbf{SA}) is effective in summarizing images within each group. Compared to average-pooling all features in each image group and use it as the group representation (Denoted as \textbf{Average} in table \ref{tab:stock} and \ref{tab:conceptual}), applying attention between images gives significant improvement. \lm{this paragraph can be merged to the last paragraph in the previous subsection}

%Our experiments demonstrate that leveraging self-attention significantly improves feature aggregation for group captioning. 
To better understand the effectiveness of self-attention, in Figure \ref{fig:attention}, we visualize the $5\times5$ self-attention weight matrix between 5 target images.
The i-th row of the attention matrix represents the attention weights from i-th image to each of the 5 images, which sum up to 1. 
In (a), images with larger and centered balloons (Image2 and Image3) gets higher attention.
In (b), image5 where the woman doing yoga is larger and easier to recognize gets higher attention.
% This indicates that each image in the group should be assigned with a different importance weight in order to get a good group representation. 
In both examples, images with more recognizable features get higher attention weights and thus contribute more to the aggregated group representation.

%and becomes the representative images of the group

%In both examples, images with more recognizable features relevant to the common content of the group get more attention and becomes the representative images of the group.

% While attention works well for summarizing the image group, directly applying attention cross two groups is not successful to capture the contrastive context-aware information(SA+CA, Atten20).
% Directly applying attention across two groups on top of self attention(SA+CA) decreases the performance largely.
% The decrease of performance can be explained because the cross attention may mix up the images from two image groups.
% To verify the influence of mixing up 2 groups, we tried directly doing one-stage attention between 20 images without separating self attention and cross attention(Atten20), which decrease the performance similarly.
% %This is a hint of disadvantage of mixing up two groups.
% %We tried adding a group embedding vector (implemented as a predefined vector, or a fully-connected layer), but this does not make significant difference either.
% However, the proposed contrastive representation is effective in contrasting the image group representation over context(SA+Contrast).
% We also tried replacing the contrastive representation with the difference of target features and reference features(SA+tgt-ref) for comparison, which improves over self-attention, but does not as significantly as the proposed methods.
% This indicates that 


% \lm{We may also need to address this question: the ground-truth is created artificially by ourselves, how do we guarantee that performing well with respect to that ground-truth translates to generating high-quality captioning? It would be best to have additional evaluation to convince that the generated caption is reasonable. Can we do a user study on this?}



\begin{table}[h!]
\small{
  \begin{center}
    \begin{tabularx}{1.01\columnwidth}{|p{3.05cm}|p{0.88cm}|X|}
        \hline
        \multicolumn{1}{|c|}{\textbf{Contrastive + Group}} & \multicolumn{1}{c}{\textbf{Group}} & \multicolumn{1}{|c|}{\textbf{Contrastive}}\\
        \hline
        \textcolor{blue}{woman} with \textcolor{red}{cowboy hat} & \textcolor{blue}{woman} & country with \textcolor{red}{cowboy} straw \textcolor{red}{hat}\\
        \hline
        %white girl & girl & white rule white and white natural green white natural chest natural wedding white natural\\
        \textcolor{red}{white} \textcolor{blue}{girl} & \textcolor{blue}{girl} & \textcolor{red}{white} rule \textcolor{red}{white} and...\\
        % \hline
        % business people in office & people & business working in working in cafe \\
        \hline
        \textcolor{blue}{woman} in \textcolor{red}{boxing glove} & \textcolor{blue}{woman} & is go in \textcolor{red}{boxing}... \\
        \hline
        \end{tabularx}
  \end{center}
  \caption{Analysis of contrastive representation. Column \texttt{Contrastive + Group} is the prediction of our full model. Column \texttt{Group} and column \texttt{Contrastive} are the predictions when only the group or only the contrastive representation is fed into the decoder respectively. \textcolor{blue}{Blue} text denotes the common part while \textcolor{red}{red} text denotes the contrastive part.}
  \label{tab:diff}
  }
\end{table}

\paragraph{Importance of multiple target and reference images.}
To investigate the effectiveness of giving multiple images in each group, we vary the number of target and reference images. 
Results are shown in Table \ref{tab:number}. 
Fewer target or reference images results in performance decline, which indicates that a larger number of images is more informational for the model to get better descriptions. 
%The decrease in performance is more sensitive to the number of target images compared to reference images, which indicates that target images play a more important role.
We also qualitatively study the importance of the reference image group. Examples are shown in Figure \ref{fig:example}. The examples indicate that when not giving reference group the predictions tend to be more generic and less discriminative.

%For example, in Figure \ref{fig:example}(b), the model without reference images generates \emph{lonely desert}, missing out \emph{tree}, which is in both target and reference groups. In another example, the model output \emph{wedding flower} without reference group, while the groundtruth is \emph{white rose}(the rose in target group is in white color while in reference groups are random colors). % The model describes \emph{women with headset} as \zemph{telephone operator} without reference group.On the other hand, given reference images, the model tends to produce more detailed description. For example, the model without reference produces \emph{olive oil} while the full model outputs \emph{olive oil bottle}.


\paragraph{Contrastive representation versus group representation.}
Table \ref{tab:diff} shows example descriptions when only the group representations or only the contrastive representations are fed into LSTM decoder. 
Although the model does not treat the features
independently and removing the features might 
break the grammar structure of the caption, 
looking at the lexicons returned by the two 
variants, we can clearly observe the focus of
two features. When the decoder uses only the group representations, the predictions emphasize the common part of two image groups. On the other hand, when the decoder only uses the contrastive representations, the predictions emphasize the difference between two image groups.
This reveals that the group representation encodes similarity information, while the contrastive representation encodes discriminative information.

% \lm{Another experiment we can do: train on Stock and test on Conceptual captioning -- with this we can show 2 things: 1. the generalization across datasets and 2. If the performance improves compared to train on Conceptual dataset, we can claim the Stock training data as a contributions.}

==> introduction.tex <==

\begin{figure}[h!]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\includegraphics[width=0.5\textwidth]{figures/1_ver3.pdf}
\end{center}
   \caption{Context-ware group captioning. Given a group of target images (shown in orange boxes) and a group of reference images which provide the context (\texttt{woman}), the goal is to generate a language description (\texttt{woman with cowboy hat}) that best describes the target group while taking into account the context depicted by the reference group.}
\label{fig:introduction}
\end{figure}

%While there has been a few works on context-based image captioning, the describing target is still single image.

%Image captioning has gained a lot of research attention in recent years.  Image captioning involves generating language description from visual data, requiring high level understanding from both language and vision. Image captioning methods have progressed rapidly in recent years thanks to advanced model for language-vision understanding. Existing image captioning methods, however, focus on describing individual images. While there has been a few works on context-based image captioning, the describing target is still single image.

Generating natural language descriptions from images, the task commonly known as image captioning, has long been an important problem in computer vision research~\cite{bai2018survey, hossain2019comprehensive, liu2019survey}.
It requires a high level of understanding from both language and vision. Image captioning has attracted a lot of research attention in recent years thanks to the advances in joint language-vision understanding models~\cite{anderson2018bottom, karpathy2015deep, rennie2017self, xu2015show}. While image captioning has progressed rapidly, existing works mostly focus on describing individual images. There are practical scenarios in which captioning images in group is desirable. Examples include summarizing personal photo albums for social sharing or understanding web user intention from their viewed or clicked images. Moreover, it is often the case that the target image group to be captioned naturally belongs to a larger set that provides the context. For instance, in text-based image retrieval applications, given a group of user-interested images and other images returned by the search engine, we could predict the user hidden preferences by contrasting the two groups and suggest a new search query accordingly. Figure~\ref{fig:introduction} shows an example of such scenario. Among all the images returned by search query \texttt{woman}, the user can indicate his/her interest in some of the images (in orange boxes). The objective is to recognize that the user wants \texttt{woman with cowboy hat} and suggest the query accordingly.

%\lm{Overall, we can emphasize more on why our proposed problem setting is important. One way to do that could be to borrow the motivation used by query suggestion papers. We can then say that: inspired by those query suggestion works in the text domain, we formulate the novel problem of "image group captioning with contrastive context"}

%This task not only has real-world applications, but is also valuable for research purpose.

%In this paper, we introduce the novel task: contrastive group captioning, which is to describe the target image group in contrastive with the reference image group.  %In the example of Figure\ref{fig:introduction}, given a group of target images(in orange box) and a group of reference images (in blue box), the task is to describe the target images in the context of reference images. This task not only has real-world applications, but is also valuable for research purpose.

%\todo{Describe the research challenge + explain why existing methods cannot be easily adapted to solve this problem: 1. There's no image captioning method for group captioning. 2. Modelling contrastive context is challenging (why?)}

Inspired by these real-world applications, we propose the novel problem of \textit{context-aware group captioning}: given a group of target images and a group of reference images, our goal is to generate a language description that best describes the target group in the context of the reference group. Compared to the conventional setting of single-image based captioning, our new problem poses two fundamental requirements. First, the captioning model needs to effectively summarize the common properties of the image groups. Second, the model needs to accurately describe the distinguishing content in the target images compared to the reference images.

To address those requirements, we develop a learning-based framework for context-aware image group captioning based on self-attention and contrastive feature construction. To obtain the feature that effectively summarizes the visual information from the image group, we develop a group-wise feature aggregation module based on self-attention. To effectively leverage the contrastive information between the target image group and the reference images, we model the context information as the aggregated feature from the whole set and subtract it from each image group feature to explicitly encourage the resulting feature to capture the differentiating properties between the target image group and the reference image group.

%The intuition of our method is to address the two subtasks: grouping the images and contrasting the images. We show that attention mechanism is successful at summarizing the images within each group. However, for contrastively capturing the difference between the two image groups, simple attention across two groups does not work well. To this end, we found negative cross attention, which is to negate the reference features before doing cross attention, improves the results. Besides, we give an case-by-case analysis showing that while attention features mainly captures similarity, subtracting the features captures the difference. 

%Another challenge is that there is no public dataset supporting this task. The required data need images to be grouped with context and be labeled with a caption that describes the whole group of images. Instead of manually labeling, we found that grouping the images by parsing results of single image captions can provide reasonably good data. We parse the single image caption into scene graphs and group the images by finding the shared scene graphs of images. However, this data generation method need the image captions to be compact and discriminative, so that they can be parsed and grouped accurately to generate clean data. To this end, we propose a large-scale compact image captioning dataset named Stock and generate data on top of it. 

Training our models requires a large number of image groups with text descriptions and associated reference image sets. In this paper, we leverage large-scale image caption datasets to construct the training data. In particular, we build our annotations on top of the Conceptual Captions~\cite{sharma2018conceptual}, a recently introduced large-scale image captioning dataset. We parse the single-image caption into scene graphs and use the shared scene graphs of image groups to generate the groups' ground-truth captions. In addition, we apply the same procedure on a large-scale image set collected from a photograph collection. This dataset contains a large number of images with compact and precise human-generated per-image descriptions. That results in our second dataset, \emph{Stock Captions}, which we plan to contribute to the research community to encourage future research in this new problem.  

%We also did experiments on public dataset Conceptual Captions\cite{sharma2018conceptual}, the data generated on top of which is not as clean as Stock. The comparison of the datasets are described in more detail in Section \ref{sec:dataset}.

Our main contributions in this paper are three-fold. First, we introduce the problem of context-aware group captioning. This novel image captioning setting can potentially be important for many real-world applications such as automatic query suggestion in image retrieval. Second, we present a learning-based approach which learns to aggregate image group visual feature for caption generation. Our framework combines the self-attention mechanism with contrastive feature construction to effectively encode the image group into a  context-aware  feature  representation, which effectively summarizes relevant common information in the groups while capturing discriminative information between the target and context group. Third, we introduce two large-scale datasets specifically for the context-aware group captioning problem. Experiments on the two datasets demonstrate that our model consistently outperforms various baselines on the context-based image group captioning task.




==> method.tex <==
\begin{figure*}
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\includegraphics[width=0.98\linewidth]{figures/3_pipeline.pdf}
\end{center}
   \caption{Method.}
\label{fig:pipeline}
\end{figure*}

In this section, we first define the task and notations. 
Then as mentioned above, we discuss methods to address the two challenges regarding this task respectively: (a) grouping, i.e, how to summarize the images within one image group, and (b) contrasting, i.e., how to figure out the difference between two image groups. 
While self-attention is effective in grouping the images, it is not as effective in contrasting.
We discuss the effectiveness of negating the reference features before attention, and thus propose to \todo{decompose ...}. 
The overall method is shown in Figure \ref{fig:pipeline}.

\subsection{Problem Setting}
Here we define the problem setting and notation formally. 
Given a group of $n_{t}$ target images and a group of $n_{r}$ reference images, our task is to generate a sentence $[w_{1}, w_{2}, ..., w_{l]}$ to describe the common features of the target image group.
Here $w_{i}$ is the word in the sentence and $l$ is sentence length, which varies for each data sample.
In our setting, $n_{t}=5, n_{r}=15$. We choose to include 20
images in one instance as the search result in a reasonable sized screen will contain roughly 20 images. The choice of number of 
images do not affect the generality of the models as
we can always sub-sample and repeat the target and reference
images.

We use ImageNet\cite{deng2009imagenet} pretrained ResNet50\cite{he2016deep} to extract features for each of the input image. 
So the input of our model are target features $\phi_{t_{1}}, ..., \phi_{t_{n_{t}}}$ and reference features $\phi_{r_{1}}, ..., \phi_{r_{n_{r}}}$, where each $\phi_{i} \in \mathbb{R}^{2048}$ is the mean-pooled feature after pool5 layer. 
While we believe that more detailed features (e.g. spatial features without mean-pooling, or object-level features) may improve performance, here We use the mean-pooled feature vector instead of spatial features in consideration of data loading speed and model training speed.
Because there are 20 images in one data sample, larger feature size will significantly increase both data loading time and training time. 
It could be a future work to explore acceleration methods, thus make using larger features possible.

\subsection{Grouping}
\subsubsection{Revisit to Transformer}
Transfomer\cite{vaswani2017attention} is a widely used attention module in natural language processing. 
The main idea is to apply attention on the input token features and thus output the context-based updated token features.
More specifically, given queries $Q$, key $K$ and values $V$, where $Q,K,V \in \mathbb{R}^{n \times d} $, transformer computes attention weights using $Q$ and $K$, and apply the weights to $V$ to update it.
$$
\text { Attention }(Q, K, V)=\operatorname{softmax}\left(\frac{Q K^{T}}{\sqrt{d}}\right) V
$$
There are trainable linear layers within the transformer module. 
Here we describe them in more detail. 
Before goes into attention kernel, each of the queries, keys and values are transformed by three linear layers, $W^Q$, $W^K$, $W^V$ respectively. 
There is a residual connection between the original values and the attention results.
After the residual connection, the result goes though two linear layers($W_{1}, b_{1}$, $W_{2}, b_{2}$) with a ReLU layer in between to get the updated result.
Another residual connection is used to add the initial attention result to the updated result.
In summary, the overall formula of transformer $F$ is:
\begin{equation*}
\begin{aligned}  
F(K, Q, V)&= V' + \max \left(0, V' W_{1}+b_{1}\right) W_{2}+b_{2} \\
V' &= V+\text { Attention }\left(Q W^{Q}, K W^{K}, V W^{V}\right) \\
\end{aligned}
\end{equation*}
An attention mask can be applied to attention weight matrix in order to remove certain attention connection.

\subsubsection{Self Attention}
Given a group of image features, we use attention to summarize them.
A naive way of grouping is average-pooling, where every image is of equal importance.
The difference between attention and naive average-pooling is that instead of summing up every image with equal weights, attention mechanism assigns different weights to each image and do weighted-sum. 
The more similar a image is with respect to all the other images in the group, the higher weight should be assigned to this image.

Following this intuition, we find that transformer, which uses inner product to compute attention weights and then apply the weights to do weighted sum, is a suitable way to group the images.
In our setting, the input keys, queries and values are concatenation of input image features $\Phi$. 
The output of transformer module is the group-based features, which is the image features updated by all the images within the group:
\begin{equation*}
\begin{aligned}  
\Phi'_{t} &= F_{st}(\Phi_{t})\\
\Phi'_{r} &= F_{sr}(\Phi_{r})
\end{aligned}
\end{equation*}
Here we simplify $F(\Phi_{t}, \Phi_{t}, \Phi_{t})$ as $F(\Phi_{t})$.
$\Phi'_{t}$ and $\Phi'_{s}$ are of the same size as $\Phi_{t}$ and $\Phi_{s}$.
We tried sharing and not sharing weights of $F_{st}$ and $F_{sr}$. 
It turns out that sharing weights lead to slightly better performance.
This can be explained that grouping target images and reference images are of no difference for the self attention module.


\subsection{Contrasting}
\subsubsection{Negative Cross Attention}
The objective of negative cross attention is to contrast target images against reference images, and vice versa. 

First, we negate the reference features. Then they are concatenated with positive features to form the input to the transformer module.
Two separate transformers are used to compute attention between each target image and every reference images and attention between each reference image and every target images.
\begin{equation*}
\begin{aligned}  
\Phi‘_{t} &= F_{ct}([\phi_{t_{1}}, ..., \phi_{t_{n_{t}}}, -\phi_{r_{1}}, ..., -\phi_{r_{n_{r}}}])\\
\Phi’_{r} &= F_{cr}([\phi_{t_{1}}, ..., \phi_{t_{n_{t}}}, -\phi_{r_{1}}, ..., -\phi_{r_{n_{r}}}])
\end{aligned}
\end{equation*}
Two masks $M_{1}, M_{2}$ are applied to the $20 \times 20$ attention weight matrix in order to mask out attention connections within each image group and only keep attention connections across two groups.

The negation operation is critical to the cross attention module. First, it results in higher attention scores between dissimilar features and lower scores for similar features. Second, it makes the resulted aggregated feature be the weighted difference , rather than the weight sum, of target and reference features.


\subsubsection{Feature Decomposing}
The updated target feature $\Phi^{s}_{t} \in \mathbb{R}^{n_{t} \times d}$ and reference feature $\Phi^{s}_{r} \in \mathbb{R}^{n_{r} \times d}$ are mean-pooled to $\phi_{t}, \phi_{r} \in \mathbb{R}^{d}$. 
Before sending them into LSTM decoder, we further decompose them into difference term $\phi_{t} - \phi_{avg}$ and common term $\phi_{s} - \phi_{avg}$, where $\phi_{avg}$ is the average of target and reference image features.
The motivation is that the former is the difference of two image groups, while the latter is the common property of the two image groups.
Then the concatenation of updated target features, updated reference features, the difference term and the common term are concatenated and feed into the LSTM decoder.
\begin{equation*}
\begin{aligned}  
\hat{w}_{1}, ..., \hat{w}_{l} = \text{LSTM}([\phi^{s}_{t}; \phi^{s}_{r}; \phi^{s}_{t} - \phi_{avg}; \phi^{s}_{r} - \phi_{avg}])
\end{aligned}
\end{equation*}
We use a standard LSTM\cite{vinyals2015show} as our decoder. While better decoder may improve the performance, we put our focus one the image feature grouping and contrasting part.


\lm{This section now has everything we need to describe in our method, which is good. I think we can restructure it a bit to make it easier for people to follow. I think we can describe our main pipeline as having 2 components: 1. feature aggregation:  given the two groups of images, we aim to obtain a compact feature representation to represent the input. For this purpose, we develop a feature aggregation module to summarize the visual feature from the two image groups into a feature vector which is then decoded into a caption.  and 2. caption generation: given an aggregated feature, a language decoder model is used to generate the caption. -- When we go into more details of the feature aggregation module, we can describe the three stages of aggregation: self-attention, negative cross attention, and decomposition.} 

==> related_work.tex <==

%{\bf image captioning} has emerged as an important research topic with a rich literature in computer vision~\cite{survey papers}. Most existing image captioning methods \cite{ordonez2011im2text, anderson2018bottom, donahue2015long, jiang2018recurrent, karpathy2015deep, rennie2017self, vinyals2015show, yao2018exploring} are based on CNN-RNN architecture (convolutional neural network and recurrent neural network\cite{hochreiter1997long}), where the visual features are extracted from CNN and fed into RNN to generate word sequence to describe the given image. Recent effort has been made towards diverse and discriminative captioning.  \cite{liu2018show, luo2018discriminability} uses the generated caption to do image retrieval and back propagate the image retrieval loss back to the image captioning model using reinforcement learning, thus supervise the caption to be more discriminative with respect to other images in the dataset. \cite{shetty2017speaking, dai2017towards} use generative adversarial networks to further supervise the captioning process. \cite{dai2017contrastive} introduces a baseline model as reference and encourages the target model to produce better distinctiveness over the baseline model. \cite{vedantam2017context} propose a decoding method that can suppress the caption elements that are common for both target image and the given distractor image. \cite{andreas2016reasoning} uses a listener to prefer the correct image over the false one. While some of the above works considered captioning on context of given distractor images the target image, there is no previous work that aims to describes a group of target images over another group of reference images. 

{\bf Image captioning} has emerged as an important research topic with a rich literature in computer vision~\cite{bai2018survey, hossain2019comprehensive, liu2019survey}. With the advances in deep neural networks, state-of-the-art image captioning approaches \cite{anderson2018bottom, donahue2015long, jiang2018recurrent, karpathy2015deep, ordonez2011im2text, rennie2017self, vinyals2015show, yao2018exploring} are based on the combination of convolutional neural networks~\cite{krizhevsky2012imagenet} and recurrent neural networks~\cite{hochreiter1997long} (CNN-RNN) architecture, where the visual features are extracted from the input image using CNNs which is then decoded by RNNs to generate the language caption describing the given image. Research in image captioning has progressed rapidly in recent years. Novel network architectures~\cite{anderson2018bottom, chen2017sca, lu2017knowing,wang2016image}, loss functions~\cite{dai2017towards, liu2017improved, liu2018show, luo2018discriminability, rennie2017self, shetty2017speaking}, and advanced joint language-vision modeling techniques~\cite{johnson2016densecap, kim2019dense, lu2017knowing, xu2015show, yang2017dense, you2016image} have been developed to enable more diverse and discriminative captioning results. Recent works have also proposed to leverage the contextual and contrastive information from additional images to help generating more distinctive caption for the target image~\cite{andreas2016reasoning, chen2018groupcap,dai2017contrastive,vedantam2017context} or comparative descriptions between image pairs~\cite{park2019robust,suhr2017corpus,suhr2018corpus,tan2019expressing}. Existing works, however, mostly focus on generating captions for a single image. Our work, on the other hand, focuses on the novel setting of context-based image group captioning which aims to describe a target image group while leveraging the context of a larger pool of reference images.

%Recent effort has been made towards diverse and discriminative captioning. \cite{liu2018show, luo2018discriminability} uses the generated caption to do image retrieval and back propagate the image retrieval loss back to the image captioning model using reinforcement learning, thus supervise the caption to be more discriminative with respect to other images in the dataset. 

{\bf Referring expression generation}~\cite{kazemzadeh2014referitgame,luo2017comprehension,yu2017joint} is a related problem to image captioning, which aims to generate natural language descriptions for a target object in an image. Contrastive modeling has been successfully applied in state-of-the-art referring expression generation methods to describe the target image region in contrast with other image regions. Yu \etal~\cite{yu2016modeling} use relative location and feature difference to discriminate the target object. Mao \etal~\cite{mao2016generation} maximize the probability of generated expression describing a specific region over other regions by Maximum Mutual Information training. While referring expression generation considers the target region in contrast with each negative region respectively, our problem requires contrastive context modeling among and between image groups.

{\bf Attention mechanism} has been successful in image captioning \cite{chen2017sca,liu2017attention, lu2017knowing, xu2015show, you2016image}. 
These works focused on applying visual attention to different spatial regions at each text generation time step.
More recently, attention in transformer\cite{vaswani2017attention} and pretrained BERT\cite{devlin2018bert} has been very successful in natural language processing tasks. 
\cite{li2019visualbert, lu2019vilbert, sun2019videobert} adapted the idea of BERT to vision and language tasks and showed improved performance on multiple sub-tasks. 
These works focus on learning attention between every word token.
In our work, we apply attention over images and show its effectiveness for summarizing information in an image group.


%{\bf Referring expression}\cite{kazemzadeh2014referitgame} aims to describe the target image region in contrast with other image regions. \cite{yu2016modeling} use relative location and feature difference to discriminate the target object.  \cite{mao2016generation} maximized the probability of generated expression describing a specific region over other regions by Maximum Mutual Information training. \cite{yu2017joint, luo2017comprehension} use a speaker-listener model where a referring expression comprehension model serves as listener. While referring expression generation considers the target region in contrast with each negative region respectively, our task target and reference are two groups of images, which has inter and intra relationships.


%{\bf Scene graph} is incorporated with image captioning and make it possible for image captioning under variants of settings. Visual Genome dataset\cite{krishna2017visual} provides dense scene graph annotation for each image, where more detailed \emph{attribute-object-relationship} annotation gives image captioning an opportunities to generate more informational descriptions. \cite{kim2019dense, yang2017dense, johnson2016densecap} densely described one image using multiple sentences, where each sentence corresponded to one object with its attributes or two objects with relationships between them.  \cite{chen2018groupcap} used visual parsing tree, which was \emph{object-relation} pairs, to select images that is similar or dissimilar with target image and thus used the similarity and dissimilarity matrix of VP-trees as additional constraint.  Motivated by their method of selecting relevant images, we choose to build the target and reference image group based on shared scene graph among images. But different from it, our problem considers multiple target and images. Considering the saliency problem, we use the scene graph parsed from image captions, rather than the densely annotated scene graph on Genome dataset.  More details are provided in Section \ref{sec:dataset}.

%\textbf{Image Contrasting}. \cite{suhr2017corpus}(NLVR) introduced the task to judge whether a given sentence describes a pair of synthetic images. \cite{suhr2018corpus}(NLVR2) extended it to real images. \cite{hu2019binary} aims to select the image that matches the given description from two candidate images. \cite{tan2019expressing, park2019robust} proposed to describe the modifications or changes between two images.

%Our setting is inspired by {\bf query suggestion}~\cite{sordoni2015hierarchical, dehghani2017learning, huang2018entity, wu2018query, jiang2018rin}, which has been studied extensively in natural language processing field. Query suggestion is a sequence prediction task, where at each timestep, the model predicts a new search query for the user given the old search query (e.g. \emph{"apple-apple phone-apple 6s"}). More recently, \cite{wu2018query} took user interaction into consideration, where user clicked documents and skipped documents at each timestep are used together with old query for the prediction of new query.  We are inspired by this task formulation and extend it to vision domain, where the clicked and skipped documents changes to target and reference image groups in our task. In this work, a memory network with attention is used to encode the sequential user clicks or skips into positive and negative memories. Because our images do not have sequential order, we use non-sequential attention to encode the two image groups.

Our setting is inspired by {\bf query suggestion}~\cite{dehghani2017learning, jiang2018rin, sordoni2015hierarchical, wu2018query} in the context of document retrieval systems. Query suggestion aims to predict the expanded query given the previous query used by the users while taking into account additional context such as search history~\cite{dehghani2017learning, jiang2018rin, sordoni2015hierarchical} or user interaction (e.g. clicked and skipped documents)~\cite{wu2018query}. We are inspired by this task formulation and extend it to vision domain. Earlier works on query suggestion in image search focus on forming visual descriptors to help obtain better search results~\cite{zha2009visual,zha2010_TOMM} while the suggested text query is obtained solely from the current user query without taking visual content understanding into account. Our work, on the other hand, can potentially be applied to enable query suggestion from images. In this work, we focus on the image captioning aspect without relying on modeling user information and behavior as in existing query suggestion works, thus making it applicable beyond retrieval tasks.

%in which our target and reference image group serve as the analogy to the clicked and skipped documents, respectively. 

%which has been studied extensively in natural language processing field. Query suggestion is a sequence prediction task, where at each timestep, the model predicts a new search query for the user given the old search query (e.g. \emph{"apple-apple phone-apple 6s"}). More recently, \cite{wu2018query} took user interaction into consideration, where user clicked documents and skipped documents at each timestep are used together with old query for the prediction of new query.  We are inspired by this task formulation and extend it to vision domain, where the clicked and skipped documents changes to target and reference image groups in our task. In this work, a memory network with attention is used to encode the sequential user clicks or skips into positive and negative memories. Because our images do not have sequential order, we use non-sequential attention to encode the two image groups.

==> related_works_cr.tex <==

%{\bf image captioning} has emerged as an important research topic with a rich literature in computer vision~\cite{survey papers}. Most existing image captioning methods \cite{ordonez2011im2text, anderson2018bottom, donahue2015long, jiang2018recurrent, karpathy2015deep, rennie2017self, vinyals2015show, yao2018exploring} are based on CNN-RNN architecture (convolutional neural network and recurrent neural network\cite{hochreiter1997long}), where the visual features are extracted from CNN and fed into RNN to generate word sequence to describe the given image. Recent effort has been made towards diverse and discriminative captioning.  \cite{liu2018show, luo2018discriminability} uses the generated caption to do image retrieval and back propagate the image retrieval loss back to the image captioning model using reinforcement learning, thus supervise the caption to be more discriminative with respect to other images in the dataset. \cite{shetty2017speaking, dai2017towards} use generative adversarial networks to further supervise the captioning process. \cite{dai2017contrastive} introduces a baseline model as reference and encourages the target model to produce better distinctiveness over the baseline model. \cite{vedantam2017context} propose a decoding method that can suppress the caption elements that are common for both target image and the given distractor image. \cite{andreas2016reasoning} uses a listener to prefer the correct image over the false one. While some of the above works considered captioning on context of given distractor images the target image, there is no previous work that aims to describes a group of target images over another group of reference images. 

{\bf Image captioning} has emerged as an important research topic with a rich literature in computer vision~\cite{bai2018survey, hossain2019comprehensive, liu2019survey}. With the advances in deep neural networks, state-of-the-art image captioning approaches \cite{anderson2018bottom, donahue2015long, jiang2018recurrent, karpathy2015deep, ordonez2011im2text, rennie2017self, vinyals2015show, yao2018exploring} are based on the combination of convolutional neural networks~\cite{krizhevsky2012imagenet} and recurrent neural networks~\cite{hochreiter1997long} (CNN-RNN) architecture, where the visual features are extracted from the input image using CNNs which is then decoded by RNNs to generate the language caption describing the given image. Research in image captioning has progressed rapidly in recent years. Novel network architectures~\cite{anderson2018bottom, chen2017sca, lu2017knowing,wang2016image}, loss functions~\cite{dai2017towards, liu2017improved, liu2018show, luo2018discriminability, rennie2017self, shetty2017speaking}, and advanced joint language-vision modeling techniques~\cite{johnson2016densecap, kim2019dense, lu2017knowing, xu2015show, yang2017dense, you2016image} have been developed to enable more diverse and discriminative captioning results. Recent works have also proposed to leverage the contextual and contrastive information from additional images to help generating more distinctive caption for the target image~\cite{andreas2016reasoning, chen2018groupcap,dai2017contrastive,vedantam2017context,huang2016visual} or comparative descriptions between image pairs~\cite{park2019robust,suhr2017corpus,suhr2018corpus,tan2019expressing}. Existing works, however, mostly focus on generating captions for a single image. Our work, on the other hand, focuses on the novel setting of context-based image group captioning which aims to describe a target image group while leveraging the context of a larger pool of reference images.

%Recent effort has been made towards diverse and discriminative captioning. \cite{liu2018show, luo2018discriminability} uses the generated caption to do image retrieval and back propagate the image retrieval loss back to the image captioning model using reinforcement learning, thus supervise the caption to be more discriminative with respect to other images in the dataset. 

{\bf Referring expression generation}~\cite{kazemzadeh2014referitgame,luo2017comprehension,yu2017joint} is a related problem to image captioning, which aims to generate natural language descriptions for a target object in an image. Contrastive modeling has been successfully applied in state-of-the-art referring expression generation methods to describe the target image region in contrast with other image regions. Yu \etal~\cite{yu2016modeling} use relative location and feature difference to discriminate the target object. Mao \etal~\cite{mao2016generation} maximize the probability of generated expression describing a specific region over other regions by Maximum Mutual Information training. While referring expression generation considers the target region in contrast with each negative region respectively, our problem requires contrastive context modeling among and between image groups.

{\bf Attention mechanism} has been successful in image captioning \cite{chen2017sca,liu2017attention, lu2017knowing, xu2015show, you2016image}. 
These works focused on applying visual attention to different spatial regions at each text generation time step.
More recently, attention in transformer\cite{vaswani2017attention} and pretrained BERT\cite{devlin2018bert} has been very successful in natural language processing tasks. 
\cite{li2019visualbert, lu2019vilbert, sun2019videobert} adapted the idea of BERT to vision and language tasks and showed improved performance on multiple sub-tasks. 
These works focus on learning attention between every word token.
In our work, we apply attention over images and show its effectiveness for summarizing information in an image group.


%{\bf Referring expression}\cite{kazemzadeh2014referitgame} aims to describe the target image region in contrast with other image regions. \cite{yu2016modeling} use relative location and feature difference to discriminate the target object.  \cite{mao2016generation} maximized the probability of generated expression describing a specific region over other regions by Maximum Mutual Information training. \cite{yu2017joint, luo2017comprehension} use a speaker-listener model where a referring expression comprehension model serves as listener. While referring expression generation considers the target region in contrast with each negative region respectively, our task target and reference are two groups of images, which has inter and intra relationships.


%{\bf Scene graph} is incorporated with image captioning and make it possible for image captioning under variants of settings. Visual Genome dataset\cite{krishna2017visual} provides dense scene graph annotation for each image, where more detailed \emph{attribute-object-relationship} annotation gives image captioning an opportunities to generate more informational descriptions. \cite{kim2019dense, yang2017dense, johnson2016densecap} densely described one image using multiple sentences, where each sentence corresponded to one object with its attributes or two objects with relationships between them.  \cite{chen2018groupcap} used visual parsing tree, which was \emph{object-relation} pairs, to select images that is similar or dissimilar with target image and thus used the similarity and dissimilarity matrix of VP-trees as additional constraint.  Motivated by their method of selecting relevant images, we choose to build the target and reference image group based on shared scene graph among images. But different from it, our problem considers multiple target and images. Considering the saliency problem, we use the scene graph parsed from image captions, rather than the densely annotated scene graph on Genome dataset.  More details are provided in Section \ref{sec:dataset}.

%\textbf{Image Contrasting}. \cite{suhr2017corpus}(NLVR) introduced the task to judge whether a given sentence describes a pair of synthetic images. \cite{suhr2018corpus}(NLVR2) extended it to real images. \cite{hu2019binary} aims to select the image that matches the given description from two candidate images. \cite{tan2019expressing, park2019robust} proposed to describe the modifications or changes between two images.

%Our setting is inspired by {\bf query suggestion}~\cite{sordoni2015hierarchical, dehghani2017learning, huang2018entity, wu2018query, jiang2018rin}, which has been studied extensively in natural language processing field. Query suggestion is a sequence prediction task, where at each timestep, the model predicts a new search query for the user given the old search query (e.g. \emph{"apple-apple phone-apple 6s"}). More recently, \cite{wu2018query} took user interaction into consideration, where user clicked documents and skipped documents at each timestep are used together with old query for the prediction of new query.  We are inspired by this task formulation and extend it to vision domain, where the clicked and skipped documents changes to target and reference image groups in our task. In this work, a memory network with attention is used to encode the sequential user clicks or skips into positive and negative memories. Because our images do not have sequential order, we use non-sequential attention to encode the two image groups.

Our setting is inspired by {\bf query suggestion}~\cite{dehghani2017learning, jiang2018rin, sordoni2015hierarchical, wu2018query} in the context of document retrieval systems. Query suggestion aims to predict the expanded query given the previous query used by the users while taking into account additional context such as search history~\cite{dehghani2017learning, jiang2018rin, sordoni2015hierarchical} or user interaction (e.g. clicked and skipped documents)~\cite{wu2018query}. We are inspired by this task formulation and extend it to vision domain. Earlier works on query suggestion in image search focus on forming visual descriptors to help obtain better search results~\cite{zha2009visual,zha2010_TOMM} while the suggested text query is obtained solely from the current user query without taking visual content understanding into account. Our work, on the other hand, can potentially be applied to enable query suggestion from images. In this work, we focus on the image captioning aspect without relying on modeling user information and behavior as in existing query suggestion works, thus making it applicable beyond retrieval tasks.

%in which our target and reference image group serve as the analogy to the clicked and skipped documents, respectively. 

%which has been studied extensively in natural language processing field. Query suggestion is a sequence prediction task, where at each timestep, the model predicts a new search query for the user given the old search query (e.g. \emph{"apple-apple phone-apple 6s"}). More recently, \cite{wu2018query} took user interaction into consideration, where user clicked documents and skipped documents at each timestep are used together with old query for the prediction of new query.  We are inspired by this task formulation and extend it to vision domain, where the clicked and skipped documents changes to target and reference image groups in our task. In this work, a memory network with attention is used to encode the sequential user clicks or skips into positive and negative memories. Because our images do not have sequential order, we use non-sequential attention to encode the two image groups.
